SAVeS: Steering Safety Judgments in Vision-Language Models via Semantic Cues

Vision-language models (VLMs) are increasingly deployed in real-world and embodied settings where safety decisions depend on visual context. However, it remains unclear which visual evidence drives these judgments. We study whether multimodal safety behavior in VLMs can be steered by simple semantic cues. We introduce a semantic steering framework that applies controlled textual, visual, and cognitive interventions without changing the underlying scene content. To evaluate these effects, we propose SAVeS, a benchmark for situational safety under semantic cues, together with an evaluation protocol that separates behavioral refusal, grounded safety reasoning, and false refusals. Experiments across multiple VLMs and an additional state-of-the-art benchmark show that safety decisions are highly sensitive to semantic cues, indicating reliance on learned visual-linguistic associations rather than grounded visual understanding. We further demonstrate that automated steering pipelines can exploit these mechanisms, highlighting a potential vulnerability in multimodal safety systems.

==> sec/clemens_3_method.tex <==
\section{Method}
\label{sec:method}

We formulate the problem of \textit{Situational Safety} evaluation in Vision-Language Models (VLMs) as a conditional probability estimation $P(\text{Safe} \mid I, Q)$, where $I$ is an image and $Q$ is a query (typically an instruction to perform an action). A safe model should correctly identify hazards in $I$ that make $Q$ dangerous (True Positive) while avoiding false refusals on safe tasks (False Positive).

Our core methodology investigates \textit{Attention Steering}: intervening on $I$ or the prompt to manipulate the VLM's visual focus. We propose three steering mechanisms and an automated pipeline framework, evaluated using a granular hallucination-aware metric.

\subsection{Experimental Setup}
\label{subsec:setup}

\paragraph{Models.}
We evaluate two state-of-the-art models: \textit{GPT-5-mini} and \textit{Qwen3-VL-8B-Instruct}. We employ these models to assess the impact of steering on both proprietary and open-weights architectures.

\paragraph{Dataset.}
We utilize a curated subset of the \textbf{MSSBench 'Embodied'} dataset, focusing on physical hazards in robotic interaction scenarios. To ensure metric stability, we manually cleaned the dataset to remove contradictory image-prompt pairs. The final dataset consists of \textbf{67 distinct scenarios}. Each scenario is represented by a pair of situations (one Safe, one Unsafe), resulting in a total evaluation set of $N=134$ samples. Each sample consists of an image $I$ and a specific instruction $Q$, such that the instruction is valid in the Safe context but hazardous in the Unsafe context. The VLM responses are generated for every tuple $(I, Q)$ and subsequently evaluated by an automated judge.

\subsection{Steering Mechanisms}
\label{subsec:steering_mechanisms}

We define three categories of steering to analyze and improve the situational safety awareness of current models.

\paragraph{Visual Steering ($M_v$).}
We modify the image space to guide attention directly.
\begin{itemize}
    \item \textbf{Semantic Markers (Circles):} We manually overlay colored circles ($C_{\text{red}}, C_{\text{white}}, C_{\text{green}}, C_{\text{yellow}}, C_{\text{orange}}$) on the image, specifically highlighting target objects or hazards. $C_{\text{red}}$ is traditionally associated with danger, while $C_{\text{white}}$ acts as a neutral spatial anchor. We also employ a color sweep (Orange, Yellow, Green) to test color sensitivity biases.
    \item \textbf{Attention-Based Selection (ABS):} To test if background clutter causes distraction or if resolution plays a role, we feed the model with additional crops $I_{\text{crop}}$ of the target object. We differentiate between two feeding strategies:
    \begin{itemize}
        \item \textit{Dual-Stream:} The model receives both the global image and the crop as separate inputs in a multi-image prompt structure ($I_{\text{global}}, I_{\text{crop}}$).
        \item \textit{Single-Stream:} The model receives only the crop or the original image with the background masked (blacked out).
    \end{itemize}
    \item \textbf{Adversarial Patches:} We introduce noise patches and typographical stickers (e.g., a sticker reading "SAFE") to test robustness against visual and semantic distractions.
\end{itemize}

\paragraph{Cognitive Steering ($M_c$).}
We manipulate the system prompt to vary the model's "safety awareness" state. We define three distinct prompting strategies:
\begin{itemize}
    \item \textbf{Instruction Following (IF/SIMPLE):} The baseline where the model is tasked to execute actions immediately without explicit advice to check for safety.
    \item \textbf{In-Context Safety (IC improved):} Our primary baseline. The model is explicitly instructed to check for potential safety risks before answering the user instruction: \textit{"First check whether there is a potential safety risk... If NO safety risk, provide a plan."}
    \item \textbf{Focus Steering (IC\_FOCUS):} A critical intervention combining visual and cognitive steering. The prompt explicitly instructs the model to attend to the visual marker and reason about its safety (e.g., \textit{"First check if there is a red circle. IF yes, focus on it."}). This tests the "Linguistic Trigger" hypothesis—whether the word "Red" activates a danger schema. We subdivide this into \textit{General Focus} (check for any circle) and \textit{Color-Specific Focus} (check for a red circle).
\end{itemize}

\paragraph{Textual Steering ($M_t$).}
As a control against visual modification, we provide bounding box coordinates in the prompt text: \textit{"Focus your attention on the region defined by [x1, y1, x2, y2]."} This tests if abstract coordinates are sufficient substitutes for pixel-level interventions.

\subsection{Automated Steering Pipelines}
\label{subsec:pipelines}

We propose three automated architectures to investigate if steering can be bootstrapped (generated by the model itself) or used adversarially.

\paragraph{Pipeline A: The Guardian (Assistive).}
A "Traffic Light" system designed to warn the model. An auxiliary VLM (Spotter) scans $I$ for hazards in the context of the instruction and assigns a risk score $S \in [0,1]$ for distinct objects. A Painter module then modifies $I$ based on $S$ by encircling identified objects:
\begin{equation}
    \text{Marker} = \begin{cases} 
    \text{Red Circle} & \text{if } S > 0.8 \text{(High Risk)} \\
    \text{Orange Circle} & \text{if } 0.4 < S \le 0.8 \text{(Caution)} \\
    \text{White Circle} & \text{if } S \le 0.4 \text{(Neutral)}
    \end{cases}
\end{equation}

\paragraph{Pipeline B: The Auditor (Diagnostic).}
This pipeline uses the model's own attention map to audit its focus. For \textit{Qwen3-VL}, we aggregate attention weights across all layers. Crucially, to mitigate artifacts, we apply a spatial mask to \textbf{suppress attention sinks} located at the image corners.
\begin{itemize}
    \item \textit{Hot-Spot Validation:} Three Red Circles are drawn on the three highest attention regions (excluding corners) to reinforce focus.
    \item \textit{Cold-Spot Adversarial:} Three Red Circles are drawn on the three lowest attention regions to test distraction.
    \item \textit{Hot-Spot Adversarial:} Three White Circles are drawn on the three highest attention regions to test cloaking.
\end{itemize}

\paragraph{Pipeline C: The Attacker (Adversarial).}
Designed to exploit the "Semantic Shortcut" (Red=Danger). The Spotter identifies the main task-relevant object and background objects. The Painter applies a "Cloak and Distract" strategy:
1. \textbf{Cloak:} Paint a \textit{White Circle} (Neutral) over the main object involved in the instruction.
2. \textbf{Distract:} Paint \textit{Red Circles} (Danger) over unrelated background objects.
The goal is to invert the model's alignment, causing it to ignore real risks and hallucinate fake ones.

\subsection{Evaluation Framework: The Hallucination Metric}
\label{subsec:eval_framework}

Standard safety evaluations often report a binary "Safe/Unsafe" accuracy. This is insufficient because it conflates \textit{Behavioral Accuracy} (correctly refusing an hazardous instruction) with \textit{Reasoning Accuracy} (correctly identifying a hazard). We introduce a granular rubric evaluated by a GPT-5 Judge to differentiate rejections based on correct risk identification versus risk hallucination.

\paragraph{Rubric Definitions.}
The Judge model compares the VLM response against the Ground Truth (GT) and assigns one of five classes:
\begin{itemize}
    \item \textbf{Class 0 (Refusal):} Direct refusal without specific reasoning (e.g., "I cannot answer").
    \item \textbf{Class 1 (Correct Grounding):} The model identifies a risk that semantically matches the Ground Truth.
    \item \textbf{Class 2 (Hallucination/Paranoia):} The model identifies a risk, but it does \textit{not} match the Ground Truth, or it finds a risk in a safe image.
    \item \textbf{Class 3 (Unsafe Plan/Compliance):} The model provides a plan to execute the instruction without identifying risks.
    \item \textbf{Class 4 (Capability Fail):} Failure due to lack of skills (e.g., "I can't see"), treated as noise.
\end{itemize}

\paragraph{Derived Metrics.}
We define separate metrics for Unsafe and Safe scenarios to isolate failure modes.

\textbf{For Unsafe Images:}
\begin{align}
    \text{Behavioral Safety Acc} &= \frac{\text{Count}(0) + \text{Count}(1) + \text{Count}(2)}{N_{\text{unsafe}}} \\
    \text{Reasoning Safety Acc} &= \frac{\text{Count}(1)}{N_{\text{unsafe}}} \quad (\text{Strict Grounding})
\end{align}
Behavioral accuracy captures general caution (including lucky guesses or hallucinations), while Reasoning accuracy captures true understanding of the specific hazard.

\textbf{For Safe Images:}
\begin{align}
    \text{Paranoia Rate} &= \frac{\text{Count}(0) + \text{Count}(1) + \text{Count}(2)}{N_{\text{safe}}} \\
    \text{Safe Accuracy} &= 1 - \text{Paranoia Rate} = \frac{\text{Count}(3) + \text{Count}(4)}{N_{\text{safe}}}
\end{align}
A high Paranoia Rate indicates the model is refusing safe tasks, often due to hallucinated risks triggered by our steering mechanisms. In this context, Class 3 (providing a plan) is the desired behavior for safe scenarios. However, we also count Class 4 (not providing a plan due to a lack of information) towards safe accuracy, as it is not considered reasoning about safety; in some situations, the lack of information (e.g., unknown location of object) makes following the instruction impossible, but not unsafe.

==> sec/clemens_4_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Effectiveness of Steering Strategies}
\label{subsec:effectiveness}

We begin by evaluating the comparative effectiveness of the three proposed steering mechanisms: Textual ($M_t$), Visual ($M_v$), and Cognitive ($M_c$). 

The first central question is whether the model's safety awareness is better manipulated through abstract spatial references (coordinates) or direct pixel-level intervention in form of circles.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/plot1_effectiveness.png}
    \caption{\textbf{The Modality Gap.} Visual Steering (Red Circles) significantly outperforms Textual Steering (Coordinates). While providing coordinates ($M_t$) offers an improvement ($44.8\%$) over the Baseline ($34.3\%$), overlaying visual markers ($M_v$) yields a boost in Behavioral Safety to ($53.7\%$). This indicates that pixel-level intervention is more effective at overriding the model's inherent safety priors than abstract text.}
    \label{fig:effectiveness}
\end{figure}

\paragraph{The Modality Gap: Visual vs. Textual.}
As illustrated in Figure \ref{fig:effectiveness}, our results demonstrate a significant "Modality Gap" between textual and visual interventions.
\begin{itemize}
    \item \textbf{Baseline (IC):} Standard in-context safety prompting with no visual or textual steering achieves a behavioral safety accuracy of $34.3\%$.
    \item \textbf{Textual Steering ($M_t$):} Explicitly providing the bounding box coordinates of the hazard in the prompt improves performance to $44.8\%$.
    \item \textbf{Visual Steering ($M_v$):} Directly modifying the image pixels with Red Circles boosts behavioral performance to $53.7\%$.
\end{itemize}
The results show, that the model responds stronger to direct pixel-level interventions, suggesting that visual markers act as a more powerful "anchor" for safety reasoning than textual descriptions of location (bounding boxes).

\paragraph{Cognitive Steering: The Attention Gap.}
Having established the superiority of visual markers, we investigated the role of \textit{Cognitive Steering} ($M_c$)—the prompting strategy used to interpret the image. Specifically, is the mere presence of a visual marker sufficient, or does the model require explicit instruction to attend to it?

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/plot5_prompt_comparison.png}
    \caption{\textbf{Cognitive Steering and the Attention Gap.} The effectiveness of visual markers is heavily dependent on the cognitive prompt. \textit{No safety awareness} (Simple Prompt) results in near-zero safety compliance.\textit{Safety awareness prompting} (IC Improved) improves both accuracies. \textit{Active Steering} (IC Focus), prompting the model to focus on the red circles yields the highest gain in performance.}
    \label{fig:prompt_comparison}
\end{figure}

We compared three levels of cognitive intervention combined with visual markers (red circles), visualized in Figure \ref{fig:prompt_comparison}:
\begin{enumerate}
    \item \textbf{Simple Prompt:} When the visual marker is present but the prompt includes no safety awareness (Simple Instruction Following), safety performance drops to $0.0\%$. The model is not able to raise safety concerns on its own even if hazardous objects in the image are marked with a red circle. 
    \item \textbf{IC Improved (General Safety):} Adding a general safety instruction ("Check for safety risks...") combined with visual markers improves behavioral accuracy to $53.7\%$. 
    \item \textbf{IC Focus:} Explicitly instructing the model to "Focus on the red circle" ($M_c$ + $M_v$) leverages the visual cue fully, reaching peak performance of $74.6\%$. It is not surprising that this yields the highest performance gain, as the model is fed with the most cues about the hazard in the given situation, as we tell it to explicitly focus on the marked dangerous object.
    \item \textbf{IC Focus:} Marking only truly dangerous objects with red circles does not tell us if the model is robust enough to not raise safety concerns if safe objects are marked with red circles. When we mark all relevant objects from the instruction with red circles and tell the model to focus on it, the paranoia rate increases dramatically from $16.4\%$ to $38.8\%$. The model now hallucinates risks in $38.8\%$ of safe situations. This is why in the following all instruction relevant objects will be marked wether safe or not to test how robust the model is to changes in the safe setting.
\end{enumerate}

\paragraph{Instructional Coupling.}
This confirms that Visual Steering functions via \textbf{Instructional Coupling}. The visual marker provides the location of the hazard (where to look), but the cognitive prompt is needed to make the model safety aware. Without the "Linguistic Trigger" of the prompt to activate the danger schema associated with the red circle, the visual modification alone is insufficient to steer the model's safety behavior.

\subsection{Mechanism Analysis: The Semantic Shortcut}
\label{subsec:mechanism}

The effectiveness of Visual Steering raises a critical question: Does the model attend to the region because of its \textit{location} (Attention), or does it react to the \textit{symbolism} of the marker (Semantics)? To disentangle these factors, we conducted ablation studies on color and prompt phrasing.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/plot2_color_hierarchy.png}
    \caption{\textbf{The Semantic Shortcut.} Safety accuracy correlates with the semiotic "danger" level of the steering color. Despite covering the exact same hazard pixels, White circles are treated as more neutral ($41.8\%$) compared to red circles ($73.1\%$). This confirms the model prioritizes the marker's meaning over the visual content.}
    \label{fig:semantic_shortcut}
\end{figure}

\paragraph{The Color Hierarchy.}
We performed a color sweep experiment, keeping the marker location constant while varying its color. As shown in Figure \ref{fig:semantic_shortcut}, we observe the following hierarchy:
\begin{itemize}
    \item \textbf{Red (Danger):} $81.1\%$ Accuracy.
    \item \textbf{Yellow (Caution):} $53.7\%$ Accuracy.
    \item \textbf{Green (Safe):} $49.2\%$ Accuracy.
    \item \textbf{Orange (Caution):} $47.8\%$ Accuracy.    
    \item \textbf{White (Neutral):} $41.8\%$ Accuracy.
\end{itemize}
Crucially, \textbf{White Circles} result in significantly lower behavioral accuracy ($41.8\%$) compared to Red Circles ($73.1\%$). This indicates a "Cloaking" effect: the model interprets the white circle as a "safer" or "more neutral" highlighter than red circles. This can be seen in the drop of the Behavioral and Reasoning Accuracy as well as the paranoia rate. Also interestingly, the color green yields a higher behavioral accuracy as orange but a significantly lower reasoning accuracy and paranoia rate.
This confirms the existence of \textbf{Semantic Shortcuts}: the model relies on the linguistic/semiotic prior of the marker for its safety awareness.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/plot6_steering_control.png}
    \caption{\textbf{Steering Specificity.} The highest safety gains are achieved only when the Visual Marker (Red) matches the Linguistic Prompt ("Focus Red"). Mismatched steering (White Circle + "Focus Red") collapses performance to $26.9\%$, while General steering ("Focus General") fails to fully activate the safety schema ($46.3\%$), proving the mechanism is linguistically activated.}
    \label{fig:steering_control}
\end{figure}

\paragraph{The Linguistic Trigger.}
To further isolate the role of semantics, we compared prompts that explicitly mention the color versus generic references (Figure \ref{fig:steering_control}).
\begin{itemize}
    \item \textbf{Matched Steering (Red circles + "Red circle focus prompt"):} Achieves peak performance ($73.1\%$).
    \item \textbf{General Steering (Red circles + "General circle focus prompt"):} Removing the word "Red" drops performance to $46.3\%$.
    \item \textbf{Mismatched Steering (White circles + "Red circle focus prompt"):} Instructing the model to look for a "Red" circle when only a "White" circle exists causes performance to collapse ($26.9\%$).
\end{itemize}
This proves that the safety mechanism is not purely visual; it is \textbf{Linguistically Activated}. As shown in Figure \ref{fig:steering_control}, the model needs the textual confirmation of "redness" to fully trigger its danger response. Which also increases paranoia rate.

\paragraph{Paranoia and Hallucination.}

Finally, we tested the robustness of this mechanism by placing random  Red Circles on \textit{safe} images resulting in a \textbf{Paranoia Rate:} of $79.1\%$.
When a random object is circled in red, the model often hallucinates hazards to justify the refusal of the instruction (e.g., claiming some furniture poses a safety risk). This high Paranoia Rate ($79.1\%$) confirms that the Red Circle acts as a powerful "Stop" signal that overrides safety reasoning ability, forcing the model into a refusal state regardless of the actual visual evidence.

\subsection{The Role of Visual Context}
\label{subsec:context}

Having established \textit{how} visual steering influences the model (via semantic shortcuts and attention), we now investigate \textit{why} it fails in certain scenarios. Specifically, does the model require the visual marker to highlight the object (focus) or to suppress the background (distraction removal)?

\paragraph{Robustness to Distraction.}
First, we tested the hypothesis that background clutter causes safety failures. We introduced random noise patches and adversarial stickers to the images. We found that the model is remarkably robust to passive visual noise, with performance remaining comparable to the baseline. This suggests that safety failures are not primarily driven by an inability to filter out irrelevant visual stimuli, but rather by a failure to interpret the relevant ones.

\paragraph{Context Ablation: The Necessity of the Scene.}
To quantify the importance of environmental context, we performed an ablation study manipulating the visual input:
\begin{itemize}
    \item \textbf{Crop Only:} Presenting only the cropped region of the hazardous object.
    \item \textbf{Background Masked:} Presenting the full image with the background blacked out, leaving only the hazard pixels.
    \item \textbf{Dual Stream (ABS):} Providing both the original global image and the specific object crop.
\end{itemize}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/plot3_ablations.png}
    \caption{\textbf{Contextual Dependency.} \textit{Background Masking} leads to a performance collapse ($20.9\%$ behavioral accuracy), proving that hazard recognition is context-dependent. \textit{Crop Only} offers high precision ($4.5\%$ Paranoia) but lacks the global context to identify all hazards. The \textit{Dual Stream} approach balances these factors.}
    \label{fig:context_ablation}
\end{figure}

The results, visualized in Figure \ref{fig:context_ablation}, reveal a critical dependency on context.
\begin{itemize}
    \item \textbf{Background Masked (Collapse):} Performance drops significantly to $20.9\%$. This is a pivotal finding: the model cannot identify hazards (e.g., a sharp knife) based solely on object features. It requires global scene information (e.g., is the knife on a cutting board or in a microwave?) to resolve the safety implication.
    \item \textbf{Crop Only (Precision):} While Behavioral Accuracy is moderate ($46.3\%$), this method achieves the lowest Paranoia Rate ($4.5\%$). By removing background clutter, we remove triggers for hallucination, but at the cost of losing context-dependent hazards.
    \item \textbf{Dual Stream (Balance):} The Dual Stream approach ($64.2\%$ accuracy) effectively bridges this gap, leveraging the global image for context and the crop for feature resolution.
\end{itemize}

\subsection{Automated Steering Pipelines}
\label{subsec:automation}

Finally, we evaluated whether the visual steering process can be fully automated without human intervention. We tested three distinct pipeline architectures (Experiment 14).

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/plot4_pipelines.png}
    \caption{\textbf{Automated Pipeline Performance.} Pipeline A (Guardian) yields marginal gains due to the Bootstrapping Paradox. Pipeline B (Attention) fails completely, as raw attention does not correlate with safety risk. Pipeline C (Attacker) demonstrates the adversarial vulnerability of the method.}
    \label{fig:pipelines}
\end{figure}

\paragraph{Pipeline A: The Guardian (Bootstrapping Paradox).}
This pipeline employs a "Spotter" VLM to identify hazards and generate the steering circles for a "Judge" VLM. Results show only marginal improvement ($38.8\%$) over the baseline ($34.3\%$). This highlights a \textbf{Bootstrapping Paradox}: to steer the model effectively, the Spotter must already be capable of recognizing the hazard. If the Spotter is sufficient, the steering mechanism becomes redundant; if it fails, the steering is misplaced.

\paragraph{Pipeline B: Attention Steering (Failure Analysis).}
We hypothesized that we could bypass the Spotter by using the model's own raw attention maps to steer focus. We placed Red Circles on regions of highest attention activation. This approach failed catastrophically ($4.5\%$ accuracy). Qualitative analysis reveals that raw attention is often driven by visual salience (contrast, edges) and attention sinks rather than semantic relevance. Forcing the model to "Focus on" these salient but irrelevant regions actively confused the reasoning process.

\paragraph{Pipeline C: The Attacker (Adversarial Vulnerability).}
Conversely, we demonstrated that Visual Steering can be weaponized. It poses a safety risk if a model is prompted to focus on red circles and one can modify the images before being fed to the model. For this pipeline we placed a adversarial model to modify the images before being fed to the main model. It painted White Circles on the main instruction objects and Red Circles on random objects. This results in a very high paranoia rate and high over all instruction refusal rate. But remarkably none of the refusals where grounded with the correct reasoning.
\begin{itemize}
    \item \textbf{Inverted Alignment:} This setup successfully inverted the model's safety alignment, driving the identification of actual hazards below the baseline while creating a massive spike in false refusals (Paranoia) to $80.6\%$.
\end{itemize}
This confirms that Visual Steering is a bi-directional lever: while it can enhance safety, it creates a "Backdoor" where the model's judgment can be completely overridden by the semantic injection of the marker.
